Remind of the Past: Incremental Learning with Analogical Prompts

Although data-free incremental learning methods are memory-friendly, accurately estimating and counteracting representation shifts is challenging in the absence of historical data. This paper addresses this thorny problem by proposing a novel incremental learning method inspired by human analogy capabilities. Specifically, we design an analogy-making mechanism to remap the new data into the old class by prompt tuning. It mimics the feature distribution of the target old class on the old model using only samples of new classes. The learnt prompts are further used to estimate and counteract the representation shift caused by fine-tuning for the historical prototypes. The proposed method sets up new state-of-the-art performance on four incremental learning benchmarks under both the class and domain incremental learning settings. It consistently outperforms data-replay methods by only saving feature prototypes for each class. It has almost hit the empirical upper bound by joint training on the Core50 benchmark. The code will be released at \url{https://github.com/ZhihengCV/A-Prompts}.

==> _macros.tex <==
%% PACKAGES (also see cvpr_header.tex)

\usepackage{times}
\usepackage{microtype}
\usepackage{epsfig}
\usepackage[table,xcdraw]{xcolor}
\usepackage{caption}
\usepackage{float}
\usepackage{placeins}
\usepackage{color, colortbl}
\usepackage{stfloats}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{xstring}
\usepackage{multirow}
\usepackage{xspace}
\usepackage{url}
\usepackage{subcaption}
\usepackage{xcolor}
\usepackage[hang,flushmargin]{footmisc}
\usepackage{bbm}

% Unfortunately, this package interferes with arxiv's stamp
\ifcamera \usepackage[accsupp]{axessibility} \fi

%% MACROS

% \newcommand{\authorname}[1]{{\textcolor{blue}{[Author: #1]}}}
% ...

% \newcommand{\commandname}{string\xspace}
% \definecolor{colorname}{rgb}{0.92,0.49,0.19}

% General

\newcommand{\nbf}[1]{{\noindent \textbf{#1.}}}

\newcommand{\supp}{supplemental material\xspace}
\ifarxiv \renewcommand{\supp}{appendix\xspace} \fi

\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}

% Reviewer commands (1 to 5), e.g. \R{1}, \R{2}
\newcommand{\R}[1]{{%
    \textbf{%
        \ifstrequal{#1}{1}{\textcolor{red}{R#1}}{%
        \ifstrequal{#1}{2}{\textcolor{blue}{R#1}}{%
        \ifstrequal{#1}{3}{\textcolor{magenta}{R#1}}{%
        \ifstrequal{#1}{4}{\textcolor{teal}{R#1}}{%
                           \textcolor{cyan}{R#1}%
        }}}}%
    }%
}}

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{2pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{packed_item}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{2pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}


==> backup/_method_back.tex <==
\section{Method}
\label{sec:method}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\x}{\boldsymbol{x}}
\newcommand{\f}{\boldsymbol{f}}
\newcommand{\p}{\boldsymbol{p}}
\newcommand{\A}{\boldsymbol{a}}
\newcommand{\B}{\boldsymbol{\varphi}}
\newcommand{\D}{\boldsymbol{\delta}}
\newcommand{\DD}{\boldsymbol{\Delta}}

\newcommand{\J}{\left[j\right]}
\newcommand{\lgt}{\boldsymbol{l}}
\newcommand{\old}{\boldsymbol{o}}
\newcommand{\new}{\boldsymbol{n}}
\newcommand{\para}{\boldsymbol{\theta}}
\newcommand{\pt}{t\!-\!1}
\newcommand{\pc}{\p_{\left\{\B^{\pt}_{y}\right\}}}
\newcommand{\xc}{\mathcal{X}^{t}_{\left\{\B^{\pt}_{y}\right\}}}

\subsection{Preliminaries and Notions}

\begin{figure*}[t] 
\centering
\includegraphics[width=0.9\linewidth]{figs/figure1.pdf} 
\caption{Schematic diagram of semantic compensation with analogous prompt.
}
\label{fig:figure1} 
\end{figure*}

\textbf{Incremental Learning}. 
Incremental learning (IL) is to train a single model on a non-stationary data stream without catastrophic forgetting. In this paper, we focus on the senior where a sequence of task is well defined, \emph{i.e.}, $t \in  \mathcal{T}=\left\{1,2,\cdots, T\right\}$, $T$ is the total task number, and we can only access the current task data. Let $\mathcal{Y}^{t}$ denote the label set of the task-$t$, and $\mathcal{S}^{t}$ denote all seen labels until the task-$t$,\emph{i.e.}, $\mathcal{S}^{t}$ = $\cup \left\{\mathcal{Y}^{1}, \mathcal{Y}^{2},...,\mathcal{Y}^{t} \right\}$. Let $\mathcal{X}^{t}$ represent the accessible samples of the task-$t$, and $(\x, y) \in \mathcal{D}^{t}$ represent the sample-label pairs of the task-$t$. $\mathcal{X}_y$ represents samples of the class-$y$. 

\textbf{Vision Transformer and Prompt Tuning}.
The vision transformer (ViT) backbone consists of two components, \emph{i.e.}, $f = f_a \circ f_e$, where $f_e$ is the embedding block which transforms the input image $\x \in \mathbb{R}^{H \times W \times C}$ into patch tokens $f_e(\x) \in \mathbb{R}^{L \times D}$, whose first token is the $[class]$ token inherited from the pretrained model; $f_a$ consists of a sequence of transformer encoders, each of which includes a multi-head attention (MHA) and a multi-layer perception (MLP). We take the first token $\f \in \mathbb{R}^{D}$ of the last layer, the corresponding output of the $[class]$ token, as the feature vector for classification tasks, \emph{i.e.}, $\f = f_a(f_e(\x))\left[1\right]$.

As $f_a$ allows arbitrary length of tokens as input, we can attach additional learnable tokens to the original image tokens, \emph{i.e.}, $f_e(\x) \oplus \p$. $\oplus$ denotes the concatenate operator along the token sequence; $\p \in \mathbb{R}^{J \times D}$ is the learnable prompt tokens, which has the same feature dimension as the image tokens. Finally, the prompt-conditioned feature vector can be calculated as $\tilde{\f}= f_a(f_e(\x) \oplus \p)\left[1\right]$, $\tilde{\f} \in \mathbb{R}^{D}$. 

In the following section, we abbreviate the above two equations as:
\begin{equation}
  \f = f_{\para}(\x), \tilde{\f} = f_{\para}(\x|\p),  
\end{equation}
where $\f$ represents the original feature vector, $\hat{\f}$ represents the prompt-conditioned feature vector, and $\para$ is the model parameters.  $f^{\pt}(\cdot)$ is the abbreviation for $f_{\para^{\pt}}(\cdot)$, which represents the model before the task-$t$ finetuning; $f^{t}(\cdot)$ is the abbreviation for $f_{\para^{t}}(\cdot)$, which represents the model after the task-$t$ finetuning. More details about ViT and prompt tuning can be found in~\cite{AlexeyDosovitskiy2020ViT,liu2021pre}, and our architecture is visualized in Fig.~\ref{}.


\subsection{Analogical Prompt Training}\label{sec:ptrain}
In this section, we describe how to train analogical prompts (A-prompts) to characterize the feature distribution of the previous seen classes with the current task's data. The training process is efficient as only the lightweight prompts need to be learnt, while the base model is frozen.

Since our method strictly follows the data-free setting, we can only save prototypes in the feature space for each old class, \emph{i.e.}, $\left\{\B_{ym}^{\pt}  | y \in \mathcal{S}^{t-1}; m \in \{1,2,\cdots,M\}  \right\}$, where $M$ is the total number saved prototypes for each class. The larger $M$ can better preserve the feature distribution, but also increases the additional memory consumption. We set $M$ to 6 in our experiments, which is comparable to the memory increase of DaulP~\cite{wang2022DualP}. We abbreviate $\B_{ym}$ in the following as $\B_{y}$ without ambiguity, because constructing and updating multiple prototypes is just a simple repetition of one prototype. We initialize prototypes with the K-Means clustering centers for each new class, and update them with the compensation method described in Sec.~\ref{sec: sdc}.

Our target is to use our A-prompts to ``convert" the new data into the old classes from the perspective of the old model, which can be measured from two aspects: first, whether the prompt-conditioned data are classified into the target class; second, whether their feature distribution is similar to the original distribution of the target class.

According to the above two criterion, we design our prompt training process. To accelerate the training of A-prompts, we first sample a subset from the current task's data $\mathcal{X}^{t}$ according their distance to the target prototype $\B^{\pt}_y, y \in \mathcal{S}^{\pt}$:
\begin{equation}\label{eq:sample}
    \xc = \left\{ \x | \x \in \mathcal{X}^{t}, f^{\pt} (\x) \in \text{K-NN}(\B^{\pt}_y) \right\}, 
\end{equation}
where $K$ is the total sample number for each historical prototype, and $\text{K-NN}(\cdot)$ is the K-Nearest-Neighbor of a given feature vector. We use these selected samples to train the prototype-specific prompts $\left\{\pc | y \in \mathcal{S}^{\pt}\right\}$, and propose an objective function includes three components:
\begin{equation}\label{eq:pt}
 \mathcal{L}_{PT} = \mathcal{L}_{CC} + \mathcal{L}_{PP} + \mathcal{L}_{DE}, \x \in \xc. 
\end{equation}

The first component is named class-convert (CC) loss, which designed to classify the prompt-conditioned data into the target old class $y \in \mathcal{S}^{\pt}$: 
\begin{equation}\label{eq:adv}
        \mathcal{L}_{CC} = -\frac{1}{N}\sum_{i=1}^{N} \log(A(h^{\pt}(\tilde{\f}^{\pt}_i))\left[ y \right]),
\end{equation}
where $N$ is the training batch size; $\tilde{\f}_{i}^{\pt} = f^{\pt}(\x_i| \p_{\left\{\B_{y}^{\pt}\right\}})$ is the prompt-conditioned feature; $h(\cdot)$ is the fully-connected classification layer; and $A(\cdot)$ is the softmax normalize function $A(\lgt)\left[j\right] = \exp(\lgt_{j})/\sum_{i}\exp(\lgt_{i})$.

The second component is named prototype-pull (PP) loss, which designed to pull the prompt-conditioned features close to the target prototype, $\cos(\cdot, \cdot)$ is the cosine similarity between two vectors: 
\begin{equation}\label{eq:pp}
    \mathcal{L}_{PP} = \frac{1}{N}\sum_{i=1}^{N}(1 - \cos(\B_{y}^{\pt}, \tilde{\f}_{i}^{\pt})).
\end{equation}

The third component is named diversity-encourage (DE) loss, which prevents prompt-conditioned features from collapsing into a single point:
\begin{equation}\label{eq:de}
    \mathcal{L}_{DE} = \frac{1}{N(N-1)}\sum_{i=1}^{N}\sum_{j=i+1}^{N}\lfloor \cos(\tilde{\f}_{i}^{\pt}, \tilde{\f}_{j}^{\pt}) - \Omega \rfloor_{+}, 
\end{equation}
where $\lfloor \cdot \rfloor_{+}$ truncates negative value to zero, $\Omega$ is a constant threshold, and we set it to $0.95$. 

Once the corresponding feature vectors of the old class for the instances of new classes are generated (prompt-conditioned feature), we can compute and then compensate for the shift of the historical prototypes, which is described in the next section.

\subsection{Analogical Feature Compensation}\label{sec: sdc}

We have ``analogized" the old classes with the A-prompts and the new data from the perspective of the old model, which to some extent equivalent to saving images of the old classes. Then, we can use these prompt-conditioned data to compensate the representation shift of the old prototypes:
\begin{equation}\label{eq:cps_p}
\begin{aligned}
  \D_i &= f^{t}(\x_i| \pc)- f^{\pt}(\x_i| \pc), \x \in \xc \\
  \DD_y &= \frac{\sum_{i} \exp( \beta \cos(f^{\pt}(\x_i| \pc), \B^{\pt}_{y})) \D_i}{\sum_{i} \exp( \beta \cos(f^{\pt}(\x_i| \pc), \B^{\pt}_{y}))}, \\
  \hat{\B}^{t}_{y} &= \B^{\pt}_{y} + \DD_{y}, 
\end{aligned}
\end{equation}
where $\D_i$ is the representation shift of the $i$-th sample, and $\DD_{y}$ is the estimated shift of $\B^{\pt}_{y}$ after the model finetuning on the task-$t$, $\beta$ is the scaling factor controls the smoothness of the above Soft-Nearest function. 

Eq.~\eqref{eq:cps_p} assumes that data points close together in the old feature space should have similar shifts after finetuning. Therefore, The reliability and the accuracy of the prototype compensation depends heavily on how close the reference data points are to this prototype. The more dense the sample points around the prototype, the more accurate the estimation of the shift will be. That's why we use Eq.~\eqref{eq:pp} to pull features towards prototypes, and use Eq.~\eqref{eq:de} to encourage the feature diversity.

\noindent \textbf{The rational of using analogical features:} SDC~\cite{LuYu2020SDC} also uses the shift compensation to update historical prototypes, Nevertheless, it directly takes the new data $\mathcal{X}^{t}$ as the reference data to calculate the shift of the old prototypes $\left\{\B^{\pt}_{y}|y \in \mathcal{S}^{\pt}\right\}$.
Theoretically, SDC performs well when there exists semantic overlaps between different tasks, performs worse when semantic gap between different tasks is enormous, since the shift direction is not consistent between distant points. This theory is also verified by our experimental results in Sec.~\ref{sec：base}. Fig.~\ref{} compare our methods with SDC. As can be seen, the original semantic gap between different classes is large, which makes the shift estimation of SDC inaccurate. Meanwhile, our method successfully remedies the semantic gap and gives more accurate shift estimations of the old prototypes.

\subsection{Model Finetuning and Classification}\label{sec:finetune}

In this section, we describe how to finetune the model on the task-$t$. For training efficiency and alleviating catastrophic forgetting , we only update MLP of each transformer encoder and the final classification header. We adopt the local softmax cross-entropy loss~\cite{masana2020class} instead of the original softmax cross-entropy loss to avoid over-penalizing historical classes, and knowledge distilling loss to maintain previous knowledge. 

We only use the new data $\mathcal{X}^{t}$ to finetune our model, without using A-prompts to ``analogize" data of old classes, because we find that distinguishing prompt-conditioned data from original ones is easy to over-fitting, and destroys the prompt-free test accuracy. 

The final objective function to finetune the model on the task-$t$ also includes three components:
\begin{equation}\label{eq:ft}
 \mathcal{L}_{FT} = \mathcal{L}_{LS} +  \mathcal{L}_{KD} + \mathcal{L}_{SC}, \x \in \mathcal{X}^{t} 
\end{equation}

The first component is named local-softmax (LS) cross-entropy loss~\cite{masana2020class}, only normalized with the new classes, which avoids over-penalizing the classes when their data is not available. $\lgt_{i}^{t} = h^{t}(f^{t}(\x_i)), \lgt_{i}^{t} \in \mathbb{R}^{|\mathcal{S}^{t}|}$ is the logits output of the new model. We can separate $\lgt^{t}$ into $\old^{t} \in \mathbb{R}^{|\mathcal{S}^{\pt}|}$, $\new^{t} \in \mathbb{R}^{|\mathcal{Y}^{t}|}$, where $\lgt^{t} = \old^{t} \oplus \new^{t}$. Finally, the classification loss is defined as follows:
\begin{equation}
    \mathcal{L}_{LS} = -\frac{1}{N}\sum_{i=1}^{N}\log(A(\new_{i}^{t})\left[y_i-|\mathcal{S}^{\pt}|\right]).
\end{equation}

The second component is the knowledge distilling (KD) loss, which is widely used in incremental learning:
\begin{equation}
  \mathcal{L}_{KD} =  -\frac{1}{N}\sum_{i=1}^{N}\sum_{j=1}^{|\mathcal{S}^{\pt}|} A\left(\lgt_{i}^{\pt}/ \zeta \right)\left[j\right]\log\left(A\left(\old_{i}^{t}/\zeta \right)\left[j\right]\right), 
\end{equation}
where $\zeta$ is the smoothing temperature, which is set to $2$ as previous methods~\cite{}. 

Moreover, we propose a shift consistency (SC) loss, which maximum the cosine similarity between and the true feature vector and the compensated feature vector:
\begin{equation}\label{eq:sc}
\begin{aligned}
  \D_j &= \f^{t}_{j} - \f^{\pt}_{j} \\
  \DD_i &= \frac{\sum_{j} \exp( \beta \cos(\f^{\pt}_{j}, \f^{\pt}_{i})) \D_j}{\sum_{j} \exp( \beta \cos(\f^{\pt}_{j}, \f^{\pt}_{i}))}, \\
  \hat{\f}^{t}_{i} &= \f^{\pt}_{i} + \DD_{i}, 
\end{aligned}
\end{equation}


\begin{equation}
 \mathcal{L}_{SC} = \frac{1}{N}\sum_{i=1}^{N} (1 - \cos(\f_{i}^{t}, \hat{\f}_{i}^{t})),  
\end{equation}
where $\f_i^{t}=f^{t}(\x_i)$ is the true feature vector of the current model, and $\hat{\f}_{i}^{t}= f^{\pt}(\x_i) + \DD_{i}$ is the compensated feature vector which uses $\left\{\x_j | j \neq i; y_{j}=y_{i}; j \in \left\{ 1,2,\cdots, N \right\} \right\}$ as the reference data to estimate $\DD_{i}$.

After finishing the model finetuning, we can easily initialize prototypes of the current task by taking the K-Means clustering centers for each new class. Then, we train A-prompts for the old prototypes by Eq.~\eqref{eq:pt}, and compensate the old prototypes by Eq.~\eqref{eq:cps_p}, which makes it possible to track prototypes along with the model update and the representation shift, More details about our training process can be found in Alg.~\ref{alg:algo_train}.  

Finally, We adopt the Soft-Nearest-Multi-Prototype (SNMP) classifier, which is an extension of  Nearest-Mean-of-Exemplars (NME) Classifier~\cite{2013distance}. NME is widely used in incremental learning~\cite{2013distance,2017icarl,LuYu2020SDC} since it can easily add novel classes by calculating their mean centers in feature space and less bias to the new classes. SNMP maintains multiple prototypes for each class instead of a single mean center, better characterizing the feature distribution and the boundary between different classes, which is formulated as follows: 
\begin{equation}\label{eq:class}
    y^* = \argmax_{y \in \mathcal{S}^{t}} \frac{\sum_{m=1}^{M} \exp(\beta \cos(f_{\para}(\x), \B_{ym}))}{\sum_{y \in \mathcal{S}^{t}}\sum_{m=1}^{M} \exp(\beta \cos(f_{\para}(\x), \B_{ym}))}.
\end{equation}



\begin{algorithm}
\caption{Model Training}\label{alg:algo_train}
\begin{footnotesize}
\KwIn{the total task number $T$; the pretrained ViT model $f$; the training sequence $\left\{\mathcal{D}^{t}|t \in \mathcal{T}\right\}$}
\KwOut{$f^{T}$; $\left\{\B^{T}_{y}|y \in \mathcal{S}^{T}\right\}$}
Initialize $f^{0}=f$;\\
\For{$t=1,\ldots,T$}{
\eIf{$t=1$}{ Train $f^{\pt}$ by $\mathcal{L}_{c}$ on $\mathcal{D}^{t}$ to get $f^{t}$; \\
             Get $\left\{\B^{t}_{y}|y \in \mathcal{Y}^{t}\right\}$ by class-wise K-Means; 
}{
    \For{$y=1,\ldots,|\mathcal{S}^{\pt}|$}{
    Sample $\xc$ by Eq.~\eqref{eq:sample}; \\
    Train $\pc$ by Eq.~\eqref{eq:pt} on $\xc$;
    }
    Training $f^{\pt}$ by Eq.~\eqref{eq:ft}  on $\mathcal{D}^{t}$ to get $f^{t}$; \\
    Get $\left\{\B^{t}_{y}|y \in \mathcal{Y}^{t}\right\}$ by class-wise K-Means; \\
    Update $\left\{\B^{\pt}_{y}|y \in \mathcal{S}^{\pt}\right\}$ to $\left\{\B^{t}_{y}|y \in \mathcal{S}^{\pt}\right\}$ in-place by Eq.~\eqref{eq:cps_p} with $\left\{(\pc, \xc)|y \in \mathcal{S}^{\pt}\right\}$ ;
}
abandon $f^{\pt}$, $\mathcal{D}^{t}$, $\left\{(\pc, \xc)|y \in \mathcal{S}^{\pt}\right\}$;
}
\Return $f^{T}$, $\left\{\B^{T}_{y}|y \in \mathcal{S}^{T}\right\}$
\end{footnotesize}
\end{algorithm}
















==> backup/_method_origin.tex <==
\section{Method}
\label{sec:method}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\x}{\boldsymbol{x}}
\newcommand{\f}{\boldsymbol{f}}
\newcommand{\p}{\boldsymbol{p}}
\newcommand{\A}{\boldsymbol{a}}
\newcommand{\B}{\boldsymbol{\varphi}}
\newcommand{\D}{\boldsymbol{\gamma}}
\newcommand{\DD}{\boldsymbol{\Gamma}}

\newcommand{\J}{\left[j\right]}
\newcommand{\lgt}{\boldsymbol{l}}
\newcommand{\old}{\boldsymbol{o}}
\newcommand{\new}{\boldsymbol{n}}
\newcommand{\para}{\boldsymbol{\theta}}
\newcommand{\pt}{t\!-\!1}
\newcommand{\pc}{\p_{\left\{\B^{\pt}_{y}\right\}}}
\newcommand{\xc}{\mathcal{X}^{t}_{\left\{\B^{\pt}_{y}\right\}}}


Incremental learning (IL) is to train a single model on a non-stationary data stream without catastrophic forgetting. In this paper, we focus on the senior where a sequence of task is well defined, \emph{i.e.}, $t \in  \mathcal{T}=\left\{1,2,\cdots, T\right\}$, $T$ is the total task number, and we can only access the current task data. Let $\mathcal{Y}^{t}$ denote the label set of the task-$t$, and $\mathcal{S}^{t}$ denote all seen label until the task-$t$,\emph{i.e.}, $\mathcal{S}^{t}$ = $\cup \left\{\mathcal{Y}^{1}, \mathcal{Y}^{2},...,\mathcal{Y}^{t} \right\}$. Let $\x \in \mathcal{X}^{t}$ represent the accessible samples, and $(\x, y) \in \mathcal{D}^{t}$ represent the sample-label pairs of the task-$t$. $\mathcal{X}_y$ represents samples in class $y$. 

\subsection{Vision Transformer and Prompt Tuning}

The vision transformer (ViT) backbone consists of two components, \emph{i.e.}, $f = f_a \circ f_e$, where $f_e$ is the embedding block which transforms the input image $\x \in \mathbb{R}^{H \times W \times C}$ into patch tokens $f_e(\x) \in \mathbb{R}^{L \times D}$, whose first token is the $[class]$ token inherited from the pretrained model; $f_a$ consists of a sequence of transformer encoders, each of which includes a multi-head attention (MHA) and a multi-layer perception (MLP). We take the first token $\f \in \mathbb{R}^{D}$ of the last layer, the corresponding output of the $[class]$ token, as the feature vector for classification tasks, \emph{i.e.}, $\f = f_a(f_e(\x))\left[1\right]$.

As $f_a$ allows arbitrary length of tokens as input, we can attach additional learnable tokens to the original image tokens, \emph{i.e.}, $f_e(\x) \oplus \p$. $\oplus$ denotes the concatenate operator along the token sequence; $\p \in \mathbb{R}^{J \times D}$ is the learnable prompt tokens, which has the same feature dimension as the image tokens. Finally, the prompt-conditioned feature vector can be calculated as $\tilde{\f}= f_a(f_e(\x) \oplus \p)\left[1\right]$, $\tilde{\f} \in \mathbb{R}^{D}$. 

In the following section, we abbreviate the above two equations as:
\begin{equation}
  \f = f_{\para}(\x), \tilde{\f} = f_{\para}(\x|\p),  
\end{equation}
where $\f$ represents the original feature vector, $\hat{\f}$ represents the prompt-conditioned feature vector, and $\para$ is the model parameters. More details about ViT and prompt tuning can be found in~\cite{}, and our network structure is visualized in Fig.~\ref{}. 

\subsection{Overall Framework}

We adopt a Soft-Nearest-Multi-Prototype (SNMP) classifier in our method, which is an extension of  Nearest-Mean-of-Exemplars (NME) Classifier~\cite{2013distance}. NME is widely used in incremental learning~\cite{2013distance,2017icarl,LuYu2020SDC} since it can easily add novel classes by calculating their mean centers in feature space. SNMP maintains multiple prototypes for each class instead of a single mean center, better characterizing the feature distribution and the boundary between different classes, which is formulated as follows: 
\begin{equation}\label{eq:class}
    y^* = \argmax_{y \in \mathcal{S}^{t}} \frac{\sum_{m=1}^{M} \exp(\beta \cos(f_{\para}(\x), \B_{ym}))}{\sum_{y \in \mathcal{S}^{t}}\sum_{m=1}^{M} \exp(\beta \cos(f_{\para}(\x), \B_{ym}))},
\end{equation}
where $\B_{ym}$ represents the $m$-th prototype of the class $y$, and $M$ is the total prototype number per class. $\cos(\cdot,\cdot)$ is the cosine similarity between two vectors, \emph{i.e.}, $\cos(\A_i, \A_j) = \frac{\A_i\cdot \A_j}{\lVert \A_i\rVert \lVert \A_j \rVert}$. $\beta$ is the scaling factor controls the softness of the classification boundary. 

After finishing the model finetuning, we can easily initialize prototypes of the current task by taking the K-Means clustering centers for each new class. The main difficulty is how to keep track of historical prototypes affected by feature drift. Previous methods~\cite{2017icarl,} solve this problem by saving a representative subsets of historical data (memory), which are used to recalculate the mean centers after finetuning. However, memory-based methods have a privacy breach risk and are memory-inefficient for long-sequence incremental learning. SDC~\cite{LuYu2020SDC} is the first data-free feature compensation method, which estimates the drift of historical prototypes with the current task data. We elaborate on its advantages and disadvantages in the following section.

\subsection{Feature Drift Compensation}

For simplicity, we abbreviate $\B_{ym}$ to $\B_{y}$ in the following sections because tracking multiple prototypes for each class is just a simple repetition of tracking one prototype.

The general feature compensation method proposed by SDC~\cite{LuYu2020SDC} assumes that data points close together in the previous feature space should have similar drift after finetuning. $f^{\pt}(\cdot)$ is the abbreviation for $f_{\para^{\pt}}(\cdot)$, which represents the model before the task-$t$ finetuning; $f^{t}(\cdot)$ is the abbreviation for $f_{\para^{t}}(\cdot)$, which represents the model after the task-$t$ finetuning. $\B^{\pt}_{y}$ is the prototype of the class-$y$ in the feature space before finetuning. SDC directly uses the current task's data $\x \in \mathcal{X}^{t}$ as the reference to estimate the compensated the historical prototype $\left\{\hat{\B}_{y}^{t}| y \in \mathcal{S}^{\pt}\right\}$:

\begin{equation}\label{eq:cps}
\begin{aligned}
  \D_i &= f^{t}(\x_i) - f^{\pt}(\x_i), \x_i \in \mathcal{X}^{t}, \\
  \DD_{y} &= \frac{\sum_{i} \exp( \beta \cos(f^{\pt}(\x_i), \B^{\pt}_{y})) \D_i}{\sum_{i} \exp( \beta \cos(f^{\pt}(\x_i), \B^{\pt}_{y}))}, \\
  \hat{\B}^{t}_{y} &= \B^{\pt}_{y} + \DD_{y}, 
\end{aligned} 
\end{equation}
where $\D_i$ is the feature drift of the $i$-th sample, and $\DD_{y}$ is the estimated feature drift of $\B^{\pt}_{y}$ after the model finetuning on the task-$t$. 

As shown in the above equation, the quality of feature drift compensation is highly dependent on whether there exists data samples near the target feature in the previous feature space. SDC assumes that there exists semantic overlaps between different tasks. However, this assumption usually cannot be met in challenging scenarios when semantic gap between different tasks is enormous, which results in bias and unreliable drift estimations. As visualized in Fig.~\ref{}, ... 

Obviously, $\mathcal{X}_y$ is the most reliable reference samples to estimate the semantic drift of $\B_y$. However, samples in previous classes are not accessible in the data-free setting. To solve this problem, we ``convert" samples from $\mathcal{X}^{t}$ to the historical classes $y \in \mathcal{S}^{\pt}$ by attaching a prototype-specific analogical prompt $\pc$.

This prompt has two effects: 1) prompt-conditioned samples will be classified into the target class corresponding to the prompt by the model before task-$t$ finetuning; 2) prompt-conditioned samples will be pulled close to the historical prototype corresponding to the prompt. Thus, the analogical prompt successfully bridge the semantic gap between the current task data with previous classes. Then, we can use these prompt-conditioned samples to estimate the semantic drift of previous prototypes more reliably. As visualized in Fig.~\ref{},...

Our method includes three stages. Firstly, we sample sample subsets from $\mathcal{X}^{t}$ according their distance to the previous prototype $\B^{\pt}_y$:
\begin{equation}\label{eq:sample}
    \xc = \left\{ \x | \x \in \mathcal{X}^{t}, f^{\pt} (\x) \in \text{K-NN}(\B^{\pt}_y) \right\},
\end{equation}
where $K$ is the total sample number for each historical prototype, and $\text{K-NN}(\cdot)$ is the K-Nearest-Neighbor of a given feature vector. We use these selected samples to train the prototype-specific prompt $\left\{\pc | y \in \mathcal{S}^{\pt}\right\}$ (details in Sec.~\ref{sec:ptrain}).

Secondly, we finetune the model with the original dataset $\mathcal{X}^{t}$ (details in Sec.~\ref{sec:finetune}), and initialize prototypes with the K-Means cluster centers for each new class.

Thirdly, We compensate previous prototypes $\hat{\B}^{t}_y=\B^{\pt}_y+\DD_y$ as the same as Eq.~\ref{eq:cps}, but with prompt-conditioned data as the reference. In particular, we use $\x_i \in \xc$ as the reference dataset, and use the prompt-conditioned transformer to replace the origin model: 
\begin{equation}\label{eq:cps_p}
\begin{aligned}
  \D_i &= f^{t}(\x_i| \pc)- f^{\pt}(\x_i| \pc), \x \in \xc \\
  \DD_y &= \frac{\sum_{i} \exp( \beta \cos(f^{\pt}(\x_i| \pc), \B^{\pt}_{y})) \D_i}{\sum_{i} \exp( \beta \cos(f^{\pt}(\x_i| \pc), \B^{\pt}_{y}))}.
\end{aligned}
\end{equation}

Finally, we use Eq.~\ref{eq:class} to classify samples in the updated feature space.  More details about our method can be in Alg.~\ref{alg:algo_train}.  

\begin{algorithm}
\caption{Model Training}\label{alg:algo_train}
\begin{footnotesize}
\KwIn{the total task number $T$; the pretrained ViT model $f$; the training sequence $\left\{\mathcal{D}^{t}|t \in \mathcal{T}\right\}$}
\KwOut{$f^{T}$; $\left\{\B^{T}_{y}|y \in \mathcal{S}^{T}\right\}$}
Initialize $f^{0}=f$;\\
\For{$t=1,\ldots,T$}{
\eIf{$t=1$}{ Train $f^{\pt}$ by $\mathcal{L}_{c}$ on $\mathcal{D}^{t}$ to get $f^{t}$; \\
             Get $\left\{\B^{t}_{y}|y \in \mathcal{Y}^{t}\right\}$ by class-wise K-Means; 
}{
    \For{$y=1,\ldots,|\mathcal{S}^{\pt}|$}{
    Sample $\xc$ by Eq.~\ref{eq:sample}; \\
    Train $\pc$ by Eq.~\ref{eq:pt} on $\xc$;
    }
    Training $f^{\pt}$ by Eq.~\ref{eq:ft}  on $\mathcal{D}^{t}$ to get $f^{t}$; \\
    Get $\left\{\B^{t}_{y}|y \in \mathcal{Y}^{t}\right\}$ by class-wise K-Means; \\
    Update $\left\{\B^{\pt}_{y}|y \in \mathcal{S}^{\pt}\right\}$ to $\left\{\B^{t}_{y}|y \in \mathcal{S}^{\pt}\right\}$ in-place by Eq.~\ref{eq:cps_p} with $\left\{(\pc, \xc)|y \in \mathcal{S}^{\pt}\right\}$ ;
}
abandon $f^{\pt}$, $\mathcal{D}^{t}$, $\left\{(\pc, \xc)|y \in \mathcal{S}^{\pt}\right\}$;
}
\Return $f^{T}$, $\left\{\B^{T}_{y}|y \in \mathcal{S}^{T}\right\}$
\end{footnotesize}
\end{algorithm}


% \begin{algorithm}
% \caption{Model Training}\label{alg:algo_train}
% \KwIn{the current task $t$; the total task number $T$; the pretrained ViT model $f$; the training data sequence $\{\mathcal{D}^{t}\}_{t=1}^{T}$}
% \KwOut{the final model $f^{T}$; the final prototypes}
% Initialize $f^{0}=f$;\\
% \For{$t=1,\ldots,T$}{
% $u^{(t)} = U_{\theta^{(t)}}(I^{(t)})$; \\
% Initialize $k=1, \beta^{(t,k)} = \mathbb{O}_{M^{t}}$; \\ 
% \tcp{$\mathbb{O}_{M^{t}} \in \mathbb{R}^{M^{t}}$ is a zero vector}
% \Repeat{$\mathcal{G}^{(t,k)}$ has converged}{
% $\mathcal{G}^{(t,k)} = \mathcal{G}(\beta^{(t,k)}, u^{(t)}, v^{(t)})$; \\ 
% \tcp{\textbf{Maximize} $\mathcal{G}$ by optimizing $\beta$}
% Update $\beta^{(t,k+1)}$ using L-BFGS;\\
% Update $k:= k+1$;
% }
% $\hat{\beta}^{(t)}=\beta^{(t,k)}$, $W_{\varepsilon}^{ub}=\mathcal{G}(\hat{\beta}^{(t)}, u^{(t)}, v^{(t)})$;\\
% \tcp{\textbf{Minimize} $W_{\varepsilon}^{ub}$ by optimizing $\theta$}
% Update $\theta^{(t+1)}$ using Adam;
% }
% \Return $\para^{T}$, 
% \end{algorithm}


\subsection{Analogical Prompt Training}\label{sec:ptrain}
We describe the prompt training stage in his section. In this stage, the only trainable parameters are analogical prompts, while other parameters are frozen. The targeted-classification loss to train  $\p_{\left\{\B_{y}^{\pt}\right\}}$ is formulated as follows:

\begin{equation}\label{eq:adv}
 \begin{aligned}   
      \tilde{\lgt}_{i}^{\pt} &= h^{\pt}(f^{\pt}(\x_i| \p_{\left\{\B_{y}^{\pt}\right\}})), \x \in \xc \\
      \mathcal{L}_{pc} &= -\frac{1}{N}\sum_{i=1}^{N} \sum_{j=1}^{|\mathcal{S}^{\pt}|} \mathbbm{1}_{\left\{j=y \right\}}\log(A(\tilde{\lgt}^{\pt}_i)\left[j\right]),
\end{aligned} 
\end{equation}
where $N$ is the training batch size, $\tilde{\lgt}^{\pt}$ is the prompt-conditioned logits output of the model before task-$t$ finetuning, $h(\cdot)$ is the fully-connected classification layer, $\mathbbm{1}_{\left\{\cdot\right\}}$ is the indicator function that equals 1 when the condition is met and 0 otherwise. $A(\cdot)$ is the softmax normalize function $A(\lgt)\left[j\right] = \frac{\exp(\lgt_{j})}{\sum_{i}\exp(\lgt_{i})}$.


The loss function defined in Eq.~\ref{eq:adv} is to distill class-specific knowledge into the analogical prompt $\p_{\left\{\B_{y}^{\pt}\right\}}$, which is further used to bridge the semantic gap between different tasks.

We also define a loss function to pull the prompt-conditioned feature vector close to the target prototype, because it's more reliable to estimate the prototype drift with nearby samples. What's more, we add a term to avoid all feature vectors collapsing into a single point: 
\begin{equation}
\begin{aligned}
    \tilde{\f}_{i}^{\pt} &= f^{\pt}(\x_i| \p_{\left\{\B_{y}^{\pt}\right\}}), \x \in \xc \\
    \mathcal{L}_{pf} &= \frac{1}{N}\sum_{i=1}^{N}(1 - \cos(\B_{y}^{\pt}, \tilde{\f}_{i}^{\pt})), \\
    \mathcal{L}_{div} &= \frac{1}{N(N-1)}\sum_{i=1}^{N}\sum_{j=i+1}^{N}\lfloor \cos(\tilde{\f}_{i}^{\pt}, \tilde{\f}_{j}^{\pt}) - \Omega \rfloor_{+}, 
\end{aligned} 
\end{equation}
where $\tilde{f}^{\pt}$ is the prompt-conditioned feature of the model before task-$t$ finetuning, $\lfloor \cdot \rfloor_{+}$ truncate negative value to zero, $\Omega$ is a constant threshold, we set it to $0.95$. 

The final objective function for training analogical prompt is defined as follows:
\begin{equation}\label{eq:pt}
 \mathcal{L}_{pt} = \mathcal{L}_{pc} + \mathcal{L}_{pf} + \mathcal{L}_{div}
\end{equation}

\subsection{Model Fintuning}\label{sec:finetune}

In this section, we describe how to finetune the model on the task-$t$. For training efficiency and alleviating catastrophic forgetting , we only update MLP of each transformer encoder and the final classification header. We adopt the local softmax cross-entropy~\cite{masana2020class} instead of the original softmax cross-entropy to avoid over-penalizing historical classes, and knowledge distilling loss to maintain previous knowledge. 

Model is training with the current task data, $x \in \mathcal{X}^{t}$, $\lgt_{i}^{t} = h^{t}(f^{t}(\x_i)), \lgt_{i}^{t} \in \mathbb{R}^{|\mathcal{S}^{t}|} $. We can separate $\lgt^{t}$ into $\old^{t} \in \mathbb{R}^{|\mathcal{S}^{\pt}|}$, $\new^{t} \in \mathbb{R}^{|\mathcal{Y}^{t}|}$, where $\lgt^{t} = \old^{t} \oplus \new^{t}$. The training objective is defined as follows: 
\begin{equation}
\begin{aligned}
  \mathcal{L}_{c} &= -\frac{1}{N}\sum_{i=1}^{N} \sum_{j=1}^{|\mathcal{Y}^{t}|}\mathbbm{1}_{\left\{j+|\mathcal{S}^{\pt}|=y_i \right\}}\log(A(\new_{i}^{t})\left[j\right]), \\
  \mathcal{L}_{d} &=  -\frac{1}{N}\sum_{i=1}^{N}\sum_{j=1}^{|\mathcal{S}^{\pt}|} A\left(\lgt_{i}^{\pt}/ \zeta \right)\left[j\right]\log\left(A\left(\old_{i}^{t}/\zeta \right)\left[j\right]\right), 
\end{aligned}
\end{equation}
where $\zeta$ is the smoothing temperature, which is set to $2$ as previous methods~\cite{}. It is worth noting that the local softmax cross-entropy is only applied to the current task's classes, which avoids over-penalizing historical classes when the historical data are unavailable. 

Moreover, we propose a drifting consistency loss, which maximum the cosine similarity between and the true feature vector and the compensated feature vector: 
\begin{equation}
 \mathcal{L}_{f} = \frac{1}{N}\sum_{i=1}^{N} (1 - \cos(\f_{i}^{t} - \hat{\f}_{i}^{t})),  
\end{equation}
where $\f_i^{t}=f^{t}(\x_i)$ is the true feature vector of the current model, and $\hat{\f}_{i}^{t}= f^{\pt}(\x_i) + \DD_{i}$ is the compensated feature vector calculated by Eq.~\ref{eq:cps} but using $\left\{\x_j | j \neq i; y_{j}=y_{i}; j \in \left\{ 1,2,\cdots, N \right\} \right\}$ as the reference data to estimate $\DD_{i}$.

The final objective function to finetune the model on the task-$t$ is defined as follows:
\begin{equation}\label{eq:ft}
 \mathcal{L}_{ft} = \mathcal{L}_{c} +  \mathcal{L}_{d} + \mathcal{L}_{f} 
\end{equation}





















==> backup/intro-backup-20221108.tex <==
\section{Introduction}
\label{sec:intro}

% 提纲:
% 第一部分首先给出增量学习的定义，明确本文不针对有task-id的情景
% 第二部分引出memory-based的设定，并对memory-based的方法不足总结
% 第三部分介绍image-sythesis的方法（额外的网络，不好训练，数据多样性得不到保证），以及特征rehearsal的方法
% 第四部分提出输入编码的概念（能不能通过当前的输入回忆起之前的知识）， 类比学习的概念并引出我们的方法
% 第五部分介绍方法，详细比较L2P Dual 以及 compensation

%  --- after training on the latest data, the performance of previously seen data degrades significantly

Incremental learning (IL), in which a single model is used to learn a non-stationary data sequence, is essential to achieve human-like AI. Many methods have been proposed to prevent \emph{catastrophic forgetting} (the significant performance degradation of previously seen data)\cite{mccloskey1989catastrophic,french1999catastrophic} during incremental learning. These methods can be roughly divided into three categories: regularization-based\cite{li2017LWF,kirkpatrick2017EWC,aljundi2018MAS,castro2018EEIL}, architecture-based\cite{yoon2017DEN,buzzega2020DER,mallya2018PackNet,mallya2018Piggyback}, and memory-based\cite{2017icarl,rolnick2019ER,Hou_2019lucir,SonglinDong2021RKD}. Most state-of-the-art methods combine at least two of them. 

Memory-based methods have superior performance in challenging scenarios where task-ID is non-accessible at inference time, such as class-incremental learning (CIL). These methods use external memory to save representative data of previous tasks and replay them during the latest training. Nonetheless, Nonetheless, concerns about memory-based methods have arisen in the community\cite{mai2022onlineSurvey,masana2020class} recently, recently, since they are susceptible to memory size and cannot be applied in scenarios with strict privacy protection and memory budget restrictions.

Data-free methods\cite{JamesSmith2021ABD,liu2022ERDR} have been proposed to avoid saving data. Several methods adopt a separate generative model to generate pseudo data of previous tasks. However, maintaining and updating an additional generative model is computationally and memory intensive and still has privacy concerns~\cite{na2018theore}. Moreover, data-free knowledge distillation~\cite{yin2020dreaming} has been introduced into incremental learning~\cite{JamesSmith2021ABD,liu2022ERDR} to avoid adding an additional generative model, which use the original classification model to optimize the random noise inputs into synthesis images. However, their performance still lags behind that of memory-based methods~\cite{JamesSmith2021ABD}. Another line of data-free methods store features rather than the original images~\cite{LuYu2020SDC,iscen2020memory} to keep previous knowledge. These methods suffers from the representation shift \XPC{that XXXX} and thus 
require estimating the drift of previously saved features with only data of the current task. It is difficult when the semantic gap between tasks is significant (details elaborated in Sec.~\ref{sec:method}). We are inspired by feature-based methods and find out the obstacle lies in how to bridge the semantic gap between different tasks. 

Our human beings depend on thinking about the relationships between things, not simply about individuals. This ability enables us to understand an infinite number of entities through associations and comparisons, and to continually learn from experience\cite{hofstadter2013Analogy}. Analogy ability has proven to be a core mechanism of human intelligence, and we can easily transform one entity to another with a simple ``prompt". For example, a motorcycle is like a cycle powered by a motor; an airport is like a port for airplanes. However, the correspondence between different entities is not always straightforward. 

In this paper, we adopt learnable, analogical prompts (a-prompts) to reparameterize data from the current classes into previously seen classes; then maintain and update previous class prototypes with these prompt-conditioned data. 

The prompt technique designs input text templates or attaches additional learnable tokens to adapt the pre-trained transformer to the downstream task rather than fine-tuning the original weights. L2P\cite{wang2022L2P} and DualPrompt\cite{wang2022DualPrompt} introduce prompt-tuning into incremental learning, maintaining a pool of prompts that convey different task information, which alleviates catastrophic forgetting caused by interference between tasks. Instead of using prompts to isolate different tasks, we use a-prompts to establish correspondence between different tasks. These prompts can be discarded after updating the model, which allows our method inference by original images without retrieving prompts from the prompt pool.

Specifically, our method consists of three stages: prompts generation, model finetuning, and prototype compensation. We use the pre-trained vision transformer (ViT)\cite{AlexeyDosovitskiy2020ViT} as our base model, the same as L2P and DualP, and adopt an additional multi-prototype nearest neighbor classifier which maintains multiple prototypes for each class to characterize the feature distribution. 

Before finetuning model on the current task's data, we first freeze the model and train a-prompts for each prototype of seen classes, the loss function includes three components: the first loss is classifying the prompt-condition data of the current task to the previous targeting class; the second loss is pulling features of prompt-condition data towards corresponding prototype; the third loss is encouraging feature diversity of the prompt-condition data to avoid trivial solution. After training, we can ``convert" the current data to any previous seen class by attaching the corresponding a-prompts.

The second stage is to finetune the model on the current task data. We only finetune each transformer encoder's multi-layer perception and the final classification header for training efficiency and alleviating catastrophic forgetting. We do not use a-prompts at this stage since distinguishing prompt-conditioned data from original ones is prone to overfitting. We adopt the local softmax cross-entropy~\cite{masana2020class} instead of the original softmax cross-entropy to avoid over-penalizing historical classes, and knowledge distilling loss to maintain previous knowledge. Moreover, we propose a drift consistency loss applied on feature space to improve our prototype compensation performance.

%  We also find that the widely used LwF method has a conflict between the knowledge distilling loss and cross-entropy loss, and we propose an improved version named LwF+, which solves the conflict by only applying cross-entropy loss on the current task.

Our prototype compensation method is inspired by Semantic drift compensation (SDC)\cite{LuYu2020SDC}. SDC first calculates the feature drifts of the current task data, i.e., the vectors pointing from the previous to the current feature space, and then estimates prototype drift using the weighted average of the data drifts, whose weights correlate negatively to distances from the data to the prototype. Finally, prototypes are updated by adding drifts to them. It assumes that data close together in the feature space should have similar drifts. This estimation is only reliable when the semantic gap between different tasks is small, i.e., some current task data are close to previous prototypes in feature space. However, in incremental learning, this condition usually is not satisfied.

To bridge the semantic gap between different tasks, instead of using the original data of the current task, we use the prompt-conditioned data already drawn close to the prototype to estimate its drift. We maintain multiple prototypes per class, initialized by k-means cluster centers and updated by prototype compensation. It is worth noting that we can drop a-prompts when the prototype update is complete. In the inference phase, we only feed original data into the model, which saves both memory and computational costs.

The contribution of this paper can be summarized as follows:
\begin{itemize}
    \item We propose analogical prompts to ``convert" the current task data into previous classes, which bridge the semantic gap between different tasks for prototype compensation.
    \item We propose a combined objective function to train diverse analogical prompts.
    \item We propose a drift consistency loss to boost performance for prototype compensation.
    \item The proposed method outperforms memory-based methods by only saving prototypes in feature space for each classes, significantly reduces additional memory and prevents privacy concerns.
	\item The proposed method achieves state-of-the-art performance on four difficult incremental learning benchmarks, including class incremental learning, domain incremental learning, and cross-domain class incremental learning. 
\end{itemize}



































